A Placement Vulnerability Study in Multi-tenant Public Clouds

Public infrastructure-as-a-service clouds, such as Amazon EC2, Google Compute Engine (GCE) and Microsoft Azure allow clients to run virtual machines (VMs) on shared physical infrastructure. This practice of multi-tenancy brings economies of scale, but also introduces the risk of sharing a physical server with an arbitrary and potentially malicious VM. Past works have demonstrated how to place a VM alongside a target victim (co-location) in early-generation clouds and how to extract secret information via side- channels. Although there have been numerous works on side-channel attacks, there have been no studies on placement vulnerabilities in public clouds since the adoption of stronger isolation technologies such as Virtual Private Clouds (VPCs). We investigate this problem of placement vulnerabilities and quantitatively evaluate three popular public clouds for their susceptibility to co-location attacks. We find that adoption of new technologies (e.g., VPC) makes many prior attacks, such as cloud cartography, ineffective. We find new ways to reliably test for co-location across Amazon EC2, Google GCE, and Microsoft Azure. We also found ways to detect co-location with victim web servers in a multi-tiered cloud application located behind a load balancer. We use our new co-residence tests and multiple customer accounts to launch VM instances under different strategies that seek to maximize the likelihood of co-residency. We find that it is much easier (10x higher success rate) and cheaper (up to $114 less) to achieve co-location in these three clouds when compared to a secure reference placement policy.

==> model_ <==

\section{Threat Model}
\label{sec:threat-model}

Co-residency attacks in public clouds, as mentioned earlier, involve two steps:
a launch strategy and co-residency detection. We assume that the adversary has
access to tools to identify a set of target victims, and either knows victim VMs' launch
characteristics or can directly trigger their launches. The latter is possible by 
increasing load in order to cause the victim to scale up by launching more instances. The focus of
this study is to identify if there exists any launch strategy that an
adversary can devise to increase the chance of co-residency with a set of
targeted victim VMs.

%%
%% We need to define placement policy in the introduction
%%

In our threat model, we assume that the cloud provider is trusted and
the attacker has no affiliation of any form with the cloud
provider. This also means that the adversary has no internal knowledge
of the placement policies that are responsible for the VM placements in
the public cloud. An adversary also has the same interface for
launching and terminated VMs as regular customers, and no other
special interfaces. Even though there may be per-account limits on the
number of VMs that a cloud provider imposes, an adversary has access
to an unlimited number of accounts and hence has no limit on the
number of VMs he could launch at any given time. 

No resource-limited cloud provider is a match to an adversary with limitless
resources and hence realistically we assume that the adversary is
resource-limited. For the same reason, a cloud provider is vulnerable
to a launch strategy only when it is trivial or cost-effective for
an adversary. As such, we aim to (i) quantify the cost of executing a launch
strategy by an adversary, (ii) define a reference placement policy with which
the placement policies of real clouds can be compared, and (iii) define
metrics to quantify a placement vulnerability as existing when there are
cost-effective launch strategies that do better than they would against the
reference policy.
%% In order to quantitatively measure a launch
%% strategy's cost-effectiveness and define placement vulnerability, we
%% need to: (i) quantify the cost of executing a launch strategy by
%% an adversary and (ii) define a reference placement policy to compare
%% various placement policies and to identify when they have a
%% vulnerability.

%\fixme{Need to define strategy $S$ more precisely}
\paragraph{Cost of a launch strategy.} Quantifying the cost of a
launch strategy is straightforward: it is the cost of launching a number of VMs and
running tests to detect co-residency with one or more target
victim VMs. To be precise, the cost of a launch strategy $S$ is given
by $C_{S} = a \cdot P(a_{type}) \cdot T_{d}(v,a)$. Here $a$ is the number of
attacker VMs of type $a_{type}$ launched to get co-located with one of
the $v$ victim VMs. $P(a_{type})$ is the price of running one VM of
type $a_{type}$ for a unit time. $T_{d}(a,v)$ is the time (in billing units) to detect
co-residency between all pairs of $a$ attackers and $v$ victim VMs, excluding pairs
within each group. %% \tnote{Why is there a subscript $d$?} \vnote{It is to
 %% indicate that it is time to ``d''etect co-residence, do you think it is distracting?}
For simplicity, we assume that the attacker is
running all instances until the last co-residency check completes or that,
equivalently. When the time to finish co-residency checks is within the
granularity of one unit of billing time (e.g., one hour on EC2), this is
equivalent to a more refined model. 

% \footnote{$T_{d}(x,y) = T_{d}(1,1) * \big( \choose{x+y}{2} -
%   \choose{x}{2} - \choose{y}{2}
%   \big)$, where $T_{d}(1,1)$ is the time taken to detect
%   co-residency
%   between a single pair of VMs.}

\paragraph{Reference placement policy.}
In order to define placement vulnerability, we need a yardstick to
compare various placement policies and the launch strategies that
they may be vulnerable to.  To aid this purpose, we define a simple
reference placement policy that has good security properties against
co-residency attacks and use it to gauge the placement policies used
in public clouds. Let there be $N$ machines in a data center and let
each machine have unlimited capacity. Given a set of unordered VM
launch requests, the mapping of each VM to a machine follows a uniform
random distribution. Let
there be $v$ victim VMs assigned to $v$ unique machines among $N$,
where $v \ll N$. The probability of {\em at least one} collision
(i.e. co-residency) under the random placement policy and the above
attack scenario when attacker launches $a$ instances is given by $1 -
\big(1-v/N\big)^a$. We call this probability the reference
probability.\footnote{This probability event follows a hypergeometric
distribution.}
  %It is the same as the
  %probability event of collision when picking two groups of balls
  %each of size $v$ and $a$ from an urn of total capacity of balls,
  %$N$.}. 
Recall that for calculating the cost of a
launch strategy under this reference policy, we also need to define
the price function, $P(vm_{type})$. For simplicity, we use the most
competitive minimum price offered by any cloud provider as the price
for the compute resource under the reference policy. %% \tnote{Why the cheapest
  %% across all clouds? We should say why we did it this way.}\vnote{The next
  %% paragraph talks about why we chose to do so.}
For example, at the time of
this study, Amazon EC2 offered t2.small instances at \$0.026 per hour of instance
activity, which was the cheapest price across all three clouds considered in
this study.


Note that the reference placement policy makes several simplifying assumptions,
but these only benefit the attacker. This is conservative as we will compare
our experimental results to the best possible launch strategy under the
reference policy. For instance, the assumption on unlimited
capacity of the servers only benefits the attacker as it never limits
the number of victim VMs an attacker could potentially co-locate
with. We use a conservative value of 1000 for $N$, which is
at least an order-of-magnitude less than the number of servers
(50,000) in the smallest reported Amazon EC2 data
centers~\cite{aws-reinvent-2014}. Similarly, the price function of
this placement policy also favors an attacker as it provides the
cheapest price possible in the market even though in reality a secure placement
policy may demand a higher price. Hence, it would be troubling if
the state-of-the-art placement policies used in public clouds does not
measure well even against such a conservative reference placement
policy.


%%  We use this reference placement policy in our experimental framework
%%  to identify placement vulnerability across cloud providers.

%% \fixme{define vulnerability in terms of cost of a strategy - compare
%%   the cost with the cost of an equivalent strategy in the reference
%%   policy achieving the same chance of coresidency.} 

\paragraph{Placement Vulnerability.} Putting it all together, we
define two metrics to gauge any launch strategy against a placement policy: (i) {\em normalized success
  rate}, and (ii) {\em cost-benefit}. The normalized success rate is the success
rate of the launch strategy in the cloud under test normalized to the success
rate of the same strategy under the reference placement policy. The cost-benefit
of a strategy is the additional cost that is incurred by the adversary in the
reference placement policy to achieve the same success rate as the strategy in the
placement policy under test. We define that a placement policy has a 
{\em placement vulnerability} if and only if there exists a launch strategy 
with a normalized success rate that is greater than 1.

\begin{figure*}[ht!]
\center
    \subfigure[GCE]{
      \includegraphics[scale=0.54]{figures/gce/gce-tr-hist.eps}
    }
    \subfigure[EC2]{
      \includegraphics[scale=0.54]{figures/ec2/ec2-tr-hist.eps}
    }
    \subfigure[Azure]{
      \includegraphics[scale=0.54]{figures/azure/azure-tr-hist.eps}
    }
    \vspace{-0.15in}
    \caption{{\bf Histogram of minimum network round trip times
        between  pairs of VMs.} The frequency is represented as a fraction
      of total number of pairs in each category. The figure does not
      show the tail of the histogram.}
    \label{fig:pings}
\end{figure*}

Note that the normalized success rate quantifies how easy it is to get
co-location. On the other hand, the cost benefit metric helps to quantify how
cheap it is to get co-location compared to a more secure placement policy. These
metrics can be used to compare launch strategies under different placement
policies, where a higher value for any of these metrics indicate that the
placement policy is relatively more vulnerable to that launch strategy. An ideal
placement policy should aim to reduce both the success rate and the cost benefit
of any strategy.

% quantify the cost benefit of any launch strategy. For example, if a
% launch strategy with $v = a = 30$ has a success rate of 0.3, the
% cost benefit of this strategy is given by the additional cost required
% to achieve the same success rate under the reference placement policy
% (which is cost equivalent of 30 instances).




==> results_ <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Placement Vulnerability Study}
\label{sec:results}

In this section, we evaluate three public clouds, Amazon EC2, Google Compute Engine
and Microsoft Azure, for placement
vulnerabilities and answer the following questions:
(i)~what are all the strategies that an adversary can employ to
increase the chance of co-location with one or more victim VMs? (ii)~what are
the chances of success and cost of each strategy? and (iii)~how do these
strategies compare against the reference placement policy
introduced in~\secref{sec:threat-model}?


%% \fixme{Need to include a general introduction to placement
%%   vulnerabilities that includes both IaaS and PaaS, mention launch
%%   strategy cost model (using a normalized pricing model) and describe
%%   PaaS results and how even \naive\ strategies are extremely cheap}

% Although, past work~\cite{rist:hey-you:ccs:2009} was done on a
% then-nascent cloud infrastructure, still provides good insights on
% range of values for the various placement parameters that we want to
% vary in our study.


% \paragraph{Experiment Setting.}
% Talk about implementation using python, libcloud api and challenges
% with azure. 


% Rewrite these details as experimental methodology

\subsection{Experimental Methodology}

Before presenting the results, we first describe the experiment setting and 
methodology that we employed for this placement vulnerability study.

\paragraph{Experiment settings.}
Recall VM placement depends on several placement variables (shown
in~\figref{fig:variables}). We assigned reasonable values to these
placement variables and enumerated through several launch
strategies. A \textit{run} corresponds to one launch strategy and
involves launching multiple VMs from two distinct accounts (i.e.,
subscriptions in Azure and projects in GCE) and checking
for co-residency between all pairs of VMs launched. One account was
designated as a proxy for the victim and the other for the adversary.
We denote a \textit{run configuration} by $v \times a$, where $v$ is the
number of victim instances and $a$ is the number of attacker instances
launched in that run. We varied $v$ and $a$ for all $v$, $a \in \{10,
20, 30\}$ and restricted them to the inequality, $v \le a$, as it increases the
likelihood of achieving co-residency.

Other placement variables that are part of the run configuration
include: victim launch time (including time of the day, day of the
week), delay between victim and attacker VM launches, victim and
attacker instance types and data center location or region where the VMs
are launched. We repeat each run multiple times across all three cloud
providers. The repetition
of experiments is especially required to control the effect of certain
environment variables like time of day. We repeat experiments for each run
configuration over various times of the day and days of the week. We
fix the instance type of VMs to small instances (t2.small on EC2,
g1.small on GCE and small or Standard-A1 on Azure) and data center
regions to us-east for EC2, us-central1-a for GCE and east-us for
Azure, unless otherwise noted. All experiments were conducted
over 3 months between December 2014 to February 2015.

%\paragraph{Local Test Machine.}
We used a single, local Intel Core i7-2600 machine with 8 SMT cores to
launch VM instances, log instance information and run the co-residency
detection test suite. 

\paragraph{Implementation and the Cloud APIs.}
In order to automate our experiments, we used Python and the
libcloud\footnote{We used libcloud version 0.15.1 for EC2, and
a modified version of 0.16.0 for GCE to support the use of multiple
accounts in GCE.} library~\cite{libcloud} to interface with EC2 and
GCE. Unfortunately, libcloud did not support Azure. The only Azure
cloud API on Linux platform was a node.js library and a cross-platform
command-line interface (CLI). We built a wrapper around the CLI. There
were no significant differences across different cloud APIs except
that Azure did not have any explicit interface to launch multiple VMs
simultaneously.

As mentioned in the experiment settings, we experimented with various
delays between the victim and attacker VM launches (0, 1, 2, 4 \ldots
hours). To save money, we reused the same set of victim instances for
each of the longer runs. That is, for the run configuration of 10x10
with 0, 1, 2, and 4 hours of delay between victim and attacker VM
launches, we launched the victim VMs only once at the start of the
experiment. After running co-residency tests on the first set of VM
pairs, we terminated all the attacker instances and relaunched
attacker VM instances after appropriate delays (say 1 hour) and rerun
the tests with {\em the same set} of victim VMs. We repeat this until
we experiment with all delays for this configuration.
We call this methodology the {\em leap-frog method}. It is also
important to note that zero delay here means parallel launch of VMs
from our test machine (and not sequential launch of VMs from one
account after another), unless otherwise noted.

In the sections below, we take a closer look at the effect of varying
one placement variable while keeping other variables fixed across
all the cloud providers. In each case, we use three metrics to measure
the degree of co-residency: chances of getting at least one
co-resident instance across a number of runs (or success rate), average number of
co-resident instances over multiple runs and average coverage
(i.e., fraction of victim VMs with which attacker VMs were
co-resident). Although these experiments were done with victim VMs
under our control, the results can be extrapolated to guide an
attacker's launch strategy for an uncooperative victim. We also
discuss a set of such strategic questions that the results help
answer. At the end of this section, we summarize and calculate the cost of
several interesting launch strategies
and evaluate the public clouds against our reference
placement policy.

% \paragraph{Reference Placement Policy.} 
% The reference placement policy assumes that there are $N$ machines in
% the datacenter, each of capacity $C$. Each of these machines can
% support $C/C_{T}$ VMs of type $T$ that has a capacity of $C_{T}$ (a
% significant fraction of the capacity of the smallest physical machine
% in the datacenter). Let $N_{T}(t)$ be the list of available slots for
% VMs of type $T$ at any given time $t$ in that datacenter. Here,
% $N_{T}(0) = N * \big(\frac{C}{C_{T}}\big)$. Note that the assumptions
% made by the reference policy are very similar to the assumptions a
% real-world task placement algorithm considers in public cluster
% management infrastructure~\cite{omega}. Given a set of VM launch
% requests, the reference placement policy places these VMs on a
% randomly chosen slot among the set of all the available slots
% $N_{T}(t)$ at that instant. Although this reference placement policy
% is simple and does not consider datacenter utilization or power
% management, it has interesting security properties against co-residency
% attacks. For instances, let there be $N$ victim instances launched at
% time, $t=0$. In order to achieve co-residency with one of $N$ VMs with
% 50\% probability, the attacker has to launch at least $\sqrt{N}$
% instances (refer to birthday paradox). A availability zone in the
% largest of all public cloud has at least 50,000 servers and can go as
% high as 300,000~\cite{aws-reinvent-2014}. Hence, for 50\% chance of
% co-residency under this reference placement startegy, an attacker has
% to launch at least 223 VMs. In reality, we find that co-residency
% happens with a significantly small number of attacker instances on the
% three public clouds under study.

\begin{figure*}
%\begin{figure}
\center
\footnotesize
\subfigure[us-central1-a]{
  \begin{tabular}{|c|c|c|c|c|c|c|}
    % \multicolumn{7}{c}{\bf GCE} \\
    \hline
    \textbf{Delay}&\textbf{Config.}& \textbf{Mean} & \textbf{S.D.} & \textbf{Min} &\textbf{Median}& \textbf{Max} \\
     (hr.) & & & & & & \\
    \hline
    0 & 10x10 & 0.11 & 0.33 & 0 & 0 & 1 \\
    0 & 10x20 & 0.2 & 0.42 & 0 & 0 & 1 \\
    0 & 10x30 & 0.5 & 0.71 & 0 & 0 & 2 \\
    0 & 20x20 & 0.43 & 0.65 & 0 & 0 & 2 \\
    0 & 20x30 & 1.67 & 1.22 & 0 & 2 & 4 \\
    0 & 30x30 & 1.6 & 1.65 & 0 & 1 & 5 \\
    1 & 10x10 & 0.25 & 0.46 & 0 & 0 & 1 \\
    1 & 10x20 & 0.33 & 0.5 & 0 & 0 & 1 \\
    1 & 10x30 & 1.6 & 1.07 & 0 & 2 & 3 \\
    1 & 20x20 & 1.27 & 1.22 & 0 & 1 & 4 \\
    1 & 20x30 & 2.44 & 1.51 & 0 & 3 & 4 \\
    1 & 30x30 & 3 & 1.12 & 1 & 3 & 5 \\
\hline
\end{tabular}
\label{tab:gce-main-nrcores}
}
 \subfigure[europe-west1-b]{
  \begin{tabular}{|c|c|c|c|c|c|c|}
    % \multicolumn{7}{c}{\bf GCE} \\
    \hline
    \textbf{Delay}&\textbf{Config.}& \textbf{Mean} & \textbf{S.D.} & \textbf{Min} &\textbf{Median}& \textbf{Max} \\
     (hr.) & & & & & & \\
    \hline
    0 & 10x10 & 2 & 1.73 & 1 & 1 & 4 \\
    0 & 10x20 & 2.67 & 1.53 & 1 & 3 & 4 \\
    0 & 10x30 & 3 & 2.65 & 1 & 2 & 6 \\
    0 & 20x20 & 3.67 & 1.53 & 2 & 4 & 5 \\
    0 & 20x30 & 2.75 & 2.06 & 0 & 3 & 5 \\
    0 & 30x30 & 12.33 & 2.08 & 10 & 13 & 14 \\
    1 & 10x10 & 2 & 1 & 1 & 2 & 3 \\
    1 & 10x20 & 2 & 1 & 1 & 2 & 3 \\
    1 & 10x30 & 2 & 1.73 & 1 & 1 & 4 \\
    1 & 20x20 & 4.67 & 5.51 & 1 & 2 & 11 \\
    1 & 20x30 & 3.75 & 2.5 & 1 & 3.5 & 7 \\
    1 & 30x30 & 10 & 3 & 7 & 10 & 13 \\
\hline
\end{tabular}
\label{tab:gce-oth-nrcores}
}
%\caption{\textbf{Distribution of number of co-resident pairs on GCE.} Region: us-central1-a.}
\caption{\textbf{Distribution of number of co-resident pairs on GCE.}}
\label{tab:gce-results}
%\label{tab:gce-main-nrcores}
\end{figure*}
%\end{figure}

% \begin{figure}
% \centering\
% \footnotesize
%   \begin{tabular}{|c|c|c|c|c|c|c|}
%     \hline
%     \textbf{Delay} (hr) & \textbf{Config} & \textbf{Mean} & \textbf{S.D.} & \textbf{Min} & \textbf{Median} & \textbf{Max} \\
%     \hline
%     0 & $*$ & 0 & 0 & 0 & 0 & 0 \\
%     % 0 & 10x20 & 0 & 0 & 0 & 0 & 0 \\
%     % 0 & 10x30 & 0 & 0 & 0 & 0 & 0 \\
%     % 0 & 20x20 & 0 & 0 & 0 & 0 & 0 \\
%     % 0 & 20x30 & 0 & 0 & 0 & 0 & 0 \\
%     % 0 & 30x30 & 0 & 0 & 0 & 0 & 0 \\
%     1 & 10x10 & 0.44 & 0.73 & 0 & 0 & 2 \\
%     1 & 10x20 & 1.11 & 1.17 & 0 & 1 & 3 \\
%     1 & 10x30 & 1.4 & 1.43 & 0 & 1.5 & 4 \\
%     1 & 20x20 & 3.57 & 2.59 & 0 & 3.5 & 9 \\
%     1 & 20x30 & 3.78 & 1.79 & 1 & 4 & 7 \\
%     1 & 30x30 & 3.89 & 2.09 & 2 & 3 & 9 \\
%     \hline
%   \end{tabular}
% \caption{\textbf{Distribution of number of co-resident pairs on
% EC2.} Region: us-east.}
% \label{tab:ec2-main-nrcores}
% \end{figure}

\begin{figure*}
\centering\
\footnotesize
\subfigure[us-east] {
  \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
    \textbf{Delay} & \textbf{Config.} & \textbf{Mean} & \textbf{S.D.} & \textbf{Min} & \textbf{Median} & \textbf{Max} \\
     (hr.) & & & & & & \\
    \hline
    0 & $*$ & 0 & 0 & 0 & 0 & 0 \\
    % 0 & 10x20 & 0 & 0 & 0 & 0 & 0 \\
    % 0 & 10x30 & 0 & 0 & 0 & 0 & 0 \\
    % 0 & 20x20 & 0 & 0 & 0 & 0 & 0 \\
    % 0 & 20x30 & 0 & 0 & 0 & 0 & 0 \\
    % 0 & 30x30 & 0 & 0 & 0 & 0 & 0 \\
    1 & 10x10 & 0.44 & 0.73 & 0 & 0 & 2 \\
    1 & 10x20 & 1.11 & 1.17 & 0 & 1 & 3 \\
    1 & 10x30 & 1.4 & 1.43 & 0 & 1.5 & 4 \\
    1 & 20x20 & 3.57 & 2.59 & 0 & 3.5 & 9 \\
    1 & 20x30 & 3.78 & 1.79 & 1 & 4 & 7 \\
    1 & 30x30 & 3.89 & 2.09 & 2 & 3 & 9 \\
    \hline
  \end{tabular}
\label{tab:ec2-main-nrcores}
}
\subfigure[us-west-1 (CA)] {
  \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
    \textbf{Delay} & \textbf{Config.} & \textbf{Mean} & \textbf{S.D.} & \textbf{Min} & \textbf{Median} & \textbf{Max} \\
     (hr.) & & & & & & \\
    \hline
    0 & $*$ & 0 & 0 & 0 & 0 & 0 \\
    0 & 20x20 & 10.33 & 8.96 & 0 & 15 & 16 \\
    1 & 10x10 & 1.67 & 0.58 & 1 & 2 & 2 \\
    1 & 10x20 & 2.33 & 0.58 & 2 & 2 & 3 \\
    1 & 10x30 & 5.33 & 2.52 & 3 & 5 & 8 \\
    1 & 20x20 & 8.33 & 4.51 & 4 & 8 & 13 \\
    1 & 20x30 & 5.5 & 3.87 & 2 & 4.5 & 11 \\
    1 & 30x30 & 8.33 & 6.66 & 4 & 5 & 16 \\
    \hline
  \end{tabular}
\label{tab:ec2-oth-nrcores}
}
\caption{\textbf{Distribution of number of co-resident pairs on
EC2.}}
\label{tab:ec2-results}
\end{figure*}


\begin{figure}
\centering\
\footnotesize
%\subfigure[Azure] {
  \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
    \textbf{Delay} (hr.) & \textbf{Config.} & \textbf{Mean} & \textbf{S.D.} & \textbf{Min} & \textbf{Median} & \textbf{Max} \\
    \hline
    0 & 10x10 & 15.22 & 19.51 & 0 & 14 & 64 \\
    0 & 10x20 & 3.78 & 4.71 & 0 & 3 & 14 \\
    0 & 10x30 & 4.25 & 6.41 & 0 & 2.5 & 19 \\
    0 & 20x20 & 9.67 & 8.43 & 0 & 8 & 27 \\
    0 & 20x30 & 2.38 & 1.51 & 1 & 2 & 5 \\
    0 & 30x30 & 24.57 & 36.54 & 1 & 6 & 99 \\
    1 & 10x10 & 2.78 & 3.87 & 0 & 1 & 12 \\
    1 & 10x20 & 0.78 & 1.2 & 0 & 0 & 3 \\
    1 & 10x30 & 0.75 & 1.39 & 0 & 0 & 3 \\
    1 & 20x20 & 0.67 & 1.66 & 0 & 0 & 5 \\
    1 & 20x30 & 0.86 & 0.9 & 0 & 1 & 2 \\
    1 & 30x30 & 4.71 & 9.89 & 0 & 1 & 27 \\
    \hline
  \end{tabular}
%}
\caption{\textbf{Distribution of number of co-resident pairs on
Azure.} Region: East US 1.}
\label{tab:azure-nrcores}
\end{figure}

\subsection{Effect of Number of Instances}
In this section, we observe the placement behavior while varying the
number of victim and attacker instances. Intuitively, we expect the
chances of co-residency to increase with the number of
attacker and victim instances. 

\begin{figure}
\center
\includegraphics[scale=0.75]{figures/all-vary-A-chance.eps}
\caption{{\bf Chances of co-residency of 10 victim instances with
varying number of attacker instances.} All these results are from one
data center region (EC2: us-east, GCE: us-central1-a, Azure: East US)
and the delays between victim and attacker instance launch were 1
hour. Results are over at least 9 runs per run configuration with at
least 3 runs per time of day.} \label{fig:vary-A-chance}

\end{figure}

\paragraph{Varying number of attacker instances.}
Keeping all the placement variables constant including the number of
victim instances, we measure the chance of co-residency over multiple
runs. The result of this experiment helps to answer the question:
How many VMs should an adversary launch to increase the chance of
co-residency?

As is shown in \figref{fig:vary-A-chance}, the placement behavior
changes across different cloud providers. For GCE and EC2, we observe
that higher the number of attacker instances relative to the victim
instances, the higher the chance of co-residency is.
\figref{tab:gce-main-nrcores} and~\ref{tab:ec2-main-nrcores} show the
distribution of number of co-resident VM pairs on GCE and EC2,
respectively. The number of co-resident VM pairs also increases with
the number of attacker instances, implying that the coverage of an
attack could be increased with larger fraction of attacker instances
than the target VM instances if the launch times are coordinated.

Contrary to our expectations, the placement behavior observed on Azure
is the inverse. The chances of co-residency with 10 attacker instances
are almost twice as high as with 30 attacker instances. This is also reflected
in the distribution of number of co-residency VM pairs (shown
in~\figref{tab:azure-nrcores}). Further investigation revealed a
correlation between the number of victim and attacker instances
launched and the chance of co-residency. That is, for the run
configuration of 10x10, 20x20 and 30x30, where number of victim and
attacker instances are the same, and with 0 delay, the chance of
co-residency were equally high for all these configurations
(between 0.9 to 1). This suggests a possible placement policy that
collates VM launch requests together based on their request size and
places them on the same group of machines.

\begin{figure}
\center
\includegraphics[scale=0.75]{figures/all-vary-V-chance.eps}
\caption{{\bf Chances of co-residency of 30 attacker instances with
varying number of victim instances.} All these
results are from one data center region (EC2: us-east, GCE:
us-central1-a, Azure: East US) and the delays between victim and
attacker instance launch were 1 hour. Results are over at least 9 runs
per run configuration with at least 3 runs per time of day.}
\label{fig:vary-V-chance}

\end{figure}


\paragraph{Varying number of victim instances.}
Similarly, we also varied the number of victim instances by keeping the number
of attacker instances and other placement variables constant (results shown
in~\figref{fig:vary-V-chance}).  We expect the chance of co-residency to
increase with the number of victims targeted. Hence, the results presented here
help an adversary answer the question: What are the chances of co-residency with
varying sizes of target victims?

As expected, we see an increase in the chances of co-residency with increasing
number of victim VMs across all cloud providers. We see that the absolute value
of the chance of co-residency is lower for Azure than other clouds. This may be
the result of significant additional delay between victim and attacker launch
times in Azure as a result of our methodology (more on this later).

\subsection{Effect of Instance Launch Time}
In this section, we answer two questions that aid an adversary to
design better launch strategies: How quickly should an attacker launch VMs
after the victim VMs are launched? Is there any increase in chance
associated with the time of day of the launch?

% Ideally, considering the reference placement policy, the chance of
% co-residency should be independent of the time of launch. But, it is
% important to notice that even the behavior of the reference model is
% dependent on the load and the churn on the system, which may be
% correlated to time of day. For instance, assuming there is spike on
% the number of VM launch request at the start (or end of the day), at
% the end of servicing all these requests the number of remaining slots
% for VMs may be drastically reduced. Subsequent VM launch requests may
% be left with a small number of avaiable slots, resulting in a
% placement behavior with increased chance of co-residency between the
% VMs that are requested after the peak request time. Thus, under the
% reference placement policy, there is no answer to the first question
% but the effect of time of day may be depedent on the churn in the
% system.

\begin{figure}
\center
\includegraphics[scale=0.75]{figures/all-vary-delay-chance.eps}
\caption{{\bf Chances of co-residency with varying delays between
victim and attacker launches.} \textit{Solid} boxes
  correspond to zero delay (simultaneous launches) and
  \textit{gauze}-like boxes correspond to 1 hour delay between victim
  and attacker launches. We did not observe any co-resident
  instances for runs with zero delay on EC2. All these results are
from one data center region (EC2: us-east, GCE: us-central1-a, Azure:
  East US). Results are over at least 9 runs per run configuration with
  at least 3 runs per time of day.}
    \label{fig:vary-delay-chance}

\end{figure}

\paragraph{Varying delay between attacker and victim launches.}
The result of varying the delay between 0 (i.e., parallel launch) and 1 hour
delay is shown in~\figref{fig:vary-delay-chance}. We can make two immediate
observations from this result.%% : in Amazon EC2 there is no chance of co-residency
%% of VMs when launched simultaneously and the placement behavior with respect
%% to the delay for GCE and Azure are inverse of each other. That is, for GCE the
%% chance of co-residency is higher with non-zero delay whereas for Azure the
%% it is higher when VMs are launched simultaneously.

\begin{figure}
\centering\
\footnotesize
% \subfigure[EC2] {
  \begin{tabular}{|c|c|c|c|c|c|c|c|}
    \hline
    \textbf{Delay} & \textbf{Mean} & \textbf{S.D.} & \textbf{Min} & \textbf{Median} & \textbf{Max} & \textbf{Success} \\
    & & & & & & \textbf{rate} \\
    \hline
    % 20x20 & Avg & SD & Min & Median & Max \\
    %0 & 0 & 0 & 0 & 0 & 0 & 0\\
    0+ & 0.6 & 1.07 & 0 & 0 & 3 & 0.30 \\
    5 min & 1.38 & 0.92 & 0 & 1 & 3 & 0.88 \\
    1 hr & 3.57 & 2.59 & 0 & 3.5 & 9 & 0.86 \\
    \hline
  \end{tabular}
%}
  \caption{\textbf{Distribution of number of co-resident pairs and success rate
      or chances of co-residency
      for shorter delays under 20x20 run configuration in EC2.} A delay with 0+
    means victim and attacker instances were launched sequentially,
    i.e. attacker instances were not launched until all victim instances were
    running. The results averaged are over 9 runs with 3 runs per time of day.}
\label{tab:ec2-short-delay}
\end{figure}

The first observation reveals a significant artifact of EC2's placement
policy: VMs launched within a short time window are never co-resident
on the same machine. This observation helps an adversary to avoid
such a strategy. We further
investigated placement behaviors on EC2 with shorter non-zero delays
in order to find the duration of this time window in which there are
zero co-residency (results shown in
~\figref{tab:ec2-short-delay}). We found that this time window is very short and
that even a sequential launch of instances (denoted by 0+)
could result in co-residency.

The second observation shows that non-zero delay on GCE and zero delay
on Azure increases the chance of co-residency and hence directly
benefits an attacker. It should be noted that on
Azure, the launch delays between victim and attacker instances were
longer than 1 hour due to our leap-frog experimental
methodology; the actual delays between the VM launches were, on
average, 3 hours (with a maximum delay of 10 hours for few runs).
This higher delay was more common in runs with larger number of
instances as there were significantly more false positives, which
required a separate sequential phase to resolve (see
\secref{ssec:coop-test}).

\begin{figure}
\center
\includegraphics[scale=0.75]{figures/long-running.eps}
\caption{{\bf Chances of co-residency over long periods.} Results include 9 runs over two
  weeks with 3 runs per time of day under 20x20 run configuration. Note that we only conducted 3 runs for 32
  hour delay as opposed to 9 runs for all other delays.}
\label{fig:long-running}
\end{figure}

We also experimented with longer delays on EC2 and
GCE to understand whether and how quickly the
chance of co-residency drops with increasing delay (results shown
in~\figref{fig:long-running}). Contrary to our expectation, we did not
find the chance of co-residency to drop to zero even for delays as high
as 16 and 32 hours. We speculate that the
reason for this observation could be that the system was under constant churn where some neighboring VMs on the
victim's machine were terminated. Note that our leap-frog methodology may,
in theory, interfere with the VM placement. But it is noteworthy that we observed
increased number of unique co-resident pairs with increasing delays, suggesting
fresh co-residency with victim VMs over longer delays. 

% \fixme{add table that shows the
%   number of co-resident pairs for a long running experiment}.


\begin{figure}
\centering\
\footnotesize
% \subfigure [GCE] { 
  \begin{tabular}{|c|c|c|c|}

    \hline
    \multicolumn{4}{|c|}{\bf Chances of Co-residency} \\
    \hline
    \textbf{Cloud} & \textbf{Morning} & \textbf{Afternoon} & \textbf{Night}\\
     & 02:00 - 10:00 & 10:00 - 18:00 & 18:00 - 02:00\\  % PST
    %& 04:00 - 12:00 & 12:00 - 20:00 & 20:00 - 04:00\\ % CST
    \hline
    %0 & 0.43 & 0.45 & 0.37 \\
    GCE & 0.68 & 0.61& 0.78 \\
    EC2 & 0.89 & 0.73 & 0.6  \\
    \hline
    % \multicolumn{4}{c}{\bf Number of Runs} \\
    % % \textbf{Delay} & \textbf{Morning} & \textbf{Afternoon} & \textbf{Night}\\
    % % & (04:00 - 12:00 CST) & (12:00 - 20:00 CST) & (20:00 - 04:00 CST)\\
    % \hline
    % 0 & 21 & 22 & 19 \\
    % 3600 & 19 & 23 & 18 \\
    % \hline

  \end{tabular}
% }
% \subfigure [EC2] { 
%   \begin{tabular}{|c|c|c|c|}

%     \hline
%     \multicolumn{4}{|c|}{\bf Chances of Coresidency} \\
%     \hline
%     \textbf{Delay} & \textbf{Morning} & \textbf{Afternoon} & \textbf{Night}\\
%     (hr) & 02:00 - 10:00 & 10:00 - 18:00 & 18:00 - 02:00\\
%     \hline
%     %0 & 0 & 0 & 0 \\
%     1 & 0.89 & 0.73 & 0.6  \\
%     \hline
%     % \multicolumn{4}{c}{\bf Number of Runs} \\
%     % % \textbf{Delay} & \textbf{Morning} & \textbf{Afternoon} & \textbf{Night}\\
%     % % & (04:00 - 12:00 CST) & (12:00 - 20:00 CST) & (20:00 - 04:00 CST)\\
%     % \hline
%     % 0 & 21 & 22 & 21 \\
%     % 3600 & 18 & 22 & 20 \\
%     % \hline

%   \end{tabular}
% }
\caption{\textbf{Effect of time of day.} Chances of
  co-residency when an attacker changes the launch time of his instances.
The results were aggregated across all run configurations with 1 hour
delay between victim and attacker launch times. All times are in PT.}
\label{tab:tod-effect} 
\end{figure}

\paragraph{Effect of time of day.}
Prior works have shown that churn or load is often correlated
with the time of day~\cite{who-was-paper}. Our simple reference
placement policy does not have a notion of load and hence have no
effect on time of day. In reality, with limited number of servers in
datacenters and limited number of capacity per host, load on the system
has direct effect on the placement behavior of any placement policy.

As expected, we observe small effect on VM placement based on the time
of day when attacker instances are launched (results shown
in~\figref{tab:tod-effect}). Specifically, there is a slightly higher
chance of co-residency if the attacker instances are launched in the
early morning for EC2 and at night for GCE.

\begin{figure}
\center
    \subfigure[GCE]{
      \includegraphics[scale=0.75]{figures/gce/gce-oth-region-cores.eps}
    }
    \subfigure[EC2]{
      \includegraphics[scale=0.75]{figures/ec2/ec2-oth-region-cores.eps}
    }
    \vspace{-0.15in}
    \caption{{\bf Median number of co-resident pairs across two
        regions.} The box plot shows the median number of co-resident
      pairs excluding co-residency within the same account. Results
      are over at least 3 run per run configuration (x-axis).}
    \label{fig:oth-nr-cores}
\end{figure}

\subsection{Effect of Data Center Location}
All the above experiments were conducted on relatively popular regions in each
cloud (especially true for EC2~\cite{who-was-paper}). In this section, we report
the results on other smaller and less popular regions.  As the regions are less
popular and have relatively fewer machines, we expect higher co-residency rates
and more co-resident instances. \figref{fig:oth-nr-cores} shows the median
number of co-resident VM pairs placed in these regions alongside the results
for popular regions. The distribution of number of co-resident instances is 
shown in~\figref{tab:gce-oth-nrcores} and~\ref{tab:ec2-oth-nrcores}.

The main observation from these experiments is that there is a higher
chance of co-residency in these smaller regions than the larger, more
popular regions. Note that we
placed at least one co-resident pair in all the runs in these
regions. Also the higher number of co-resident pairs also suggests a
larger coverage over victim VMs in these smaller regions.

One anomaly that we found during two 20x20 runs on EC2 between
$30^{th}$ and $31^{st}$ of January 2015, when we observed an unusually
large number of co-resident instances (including three VMs from the
same account). We believe this anomaly may be a result of an internal
management incident in the Amazon EC2 us-west-1 region.

\begin{figure}
\center
\includegraphics[scale=0.75]{figures/azure/azure-cores-hist.eps}
\caption{{\bf Distribution of number of co-resident instances per host on
    Azure.} The results shown are across all the runs. We saw at most 2
  instances per host in EC2 and at most 3 instances per host in GCE.}
  % Each group of co-resident node is counted only once towards
  % the highest number of co-resident nodes (e.g. 3 node group is not
  % counted again 3 times as a 2-node group of co-resident nodes).
\label{fig:azure-cores}

\end{figure}

\subsection{Other Observations}

We report several other interesting observations in this section.
First, we found more than two VMs can be co-resident on the same host
on both Azure and GCE, but not on EC2. \figref{fig:azure-cores} shows the
distribution of number of co-resident instances per host.
Particularly, in one of the runs, we placed 16 VMs on a single
host.

Another interesting observation is related to co-resident instances
from the same account. We term them as {\em self-co-resident instances}.
We observed many self-co-resident pairs on GCE and Azure
(not shown). On the other hand, we never noticed any self co-resident
pair on EC2 except for the anomaly in us-west-1. Although we did not
notice any effect on the actual chance of co-residence, we believe
such placement behaviors (or the lack of) may affect VM placement.

We also experimented with medium instances and successfully placed few
co-located VMs on both EC2 and GCE by employing similar successful strategies
learned with small instances.

%%
%% Things that we do not report in this submission
%%

% note on self coresident instances and that there were none on EC2
% and its implications
% azure coresident instances per host
% single VM tests


\subsection{Cost of Launch Strategies}
\begin{figure}
\center
\includegraphics[scale=0.75]{figures/all-test-duration.eps}
\vspace{-0.2in}
\caption{{\bf Launch strategy and co-residency detection execution
    times.} The run configurations $v \times a$ indicates the number of
  victims vs. number of attackers launched. The error bars show the
  standard deviation across at least 7 runs.}
    \label{fig:test-duration}
\end{figure}


\begin{figure}
  \center
  \footnotesize
  \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
    {\bf Run} & \multicolumn{3}{c|}{\bf Average Cost (\$)} & \multicolumn{3}{c|}{\bf Maximum Cost (\$)} \\
    {\bf config.} & GCE & EC2 & Azure & GCE & EC2 & Azure\\
    \hline
    10x10 & \textbf{0.137} & 0.260 & 0.494 & 0.140 & 0.260 & 0.819\\
    10x20 & 0.370 & 0.520 & 1.171 & 0.412 & 0.520 & 1.358\\
    10x30 & 1.049 & 0.780 & 2.754 & 1.088 & 1.560 & 3.257\\
    20x20 & 0.770 & 0.520 & 2.235 & 1.595 & 1.040 & 3.255\\
    20x30 & 1.482 & 1.560 & 3.792 & 1.581 & 1.560 & 4.420\\
    30x30 & 1.866 & 1.560 & 5.304 & 2.433 & 1.560 & \textbf{7.965}\\
    \hline
  \end{tabular}
  \caption{\textbf{Cost of running a launch strategy} (in
    dollars). Maximum cost column refers to the maximum cost we
    incurred out of all the runs for that particular configuration and
    cloud provider. The cost per hour of small
    instances at the time of this study were: 0.05, 0.026 and 0.06
    dollars for GCE, EC2 and Azure, respectively. The minimum and
    maximum costs are in \textbf{bold}.}
\label{tab:cost-strategies}
\end{figure}

Recall that the cost of a launch strategy from
\secref{sec:threat-model}, $C_{S} = a * P(a_{type}) * T_{d}(v,a)$. In
order to calculate this cost, we need $T_{d}(v,a)$ which is the time
taken to detect co-location with $a$ attackers and $v$
victims. \figref{fig:test-duration} shows the average time taken to
complete launching attacker instances and complete co-residency detection
for each run configuration. Here the measured co-residency detection
is the parallelized version discussed in \secref{ssec:coop-test} and
also includes time taken to detect co-residency within each tenant
account. Hence, for these reasons the time to detect co-location is an
upper bound for a realistic and highly optimized co-residency
detection mechanism. 

We calculate the cost of executing each launch strategy under the
three public clouds. The result is summarized
in~\figref{tab:cost-strategies}. Note that we only consider the cost
incurred by the compute instances because the cost for
other resources such as network and storage, was insignificant. Also note
that EC2 bills every hour even if an instance runs less than an
hour~\cite{ec2-pricing}, whereas GCE and Azure charge per minute of
instance activity. This difference is considered in our cost
calculation. Overall, the maximum cost
we incurred was about \$8 for running 30 VMs for 4 hours 25 minutes on
Azure and a minimum of 14 cents on GCE for running 10 VMs for 17
minutes. We incurred the highest cost for all the launch strategies in
Azure because of overall higher cost per hour and partly due to longer tests due to our
co-residency detection methodology. 
%\fixme{Say why Azure higher: cost more per minute, lower perf ratio caused longer tests}

\subsection{Summary of Placement Vulnerabilities}

%\fixme{Include discussion on cost of each strategy}

\noindent In this section, we return to the secure reference placement policy
introduced in \secref{sec:threat-model} and use it to identify placement
vulnerabilities across all the three clouds. Recall that the probability of at
least one pair of co-residency under this random placement policy is given by
%$\Prob{\E_{a}^{v} > 0} = 1 - \Big( \frac{N - v}{N} \Big)^a$,
$\Prob{\E_{a}^{v} > 0} = 1 - (1 - v/N)^a$, where $\E_{a}^{v}$ is the random
variable denoting the number of co-location observed when placing $a$ attacker
VMs among $N=1000$ total machines where $v$ machines are already picked for the
$v$ victim VMs. First, we evaluate this
probability for various run configurations that we experimented with in the
public clouds. The probabilities are shown in~\figref{fig:ref-mode-prob}.

%\begin{figure}
%  \center
%  \footnotesize
%    \begin{tabular}{|c|c|}
%    \hline
%    \textbf{Run Config.} & $ \Prob{\E_{a}^{v} > 0}$ \\
%    \hline
%    10x10 & 0.10 \\
%    10x20 & 0.18 \\
%    10x30 & 0.26 \\
%    20x20 & 0.33 \\
%    20x30 & 0.45 \\
%    30x30 & 0.60 \\
%    \hline
%  \end{tabular}
%  \caption{\textbf{Probability of co-residency under the reference
%      placement policy.}}
%  \label{fig:ref-mode-prob}
%\end{figure}

\begin{figure}
  \center
  \footnotesize
    \begin{tabular*}{\columnwidth}{c|cccccc}
    \hline
    \textbf{Run Config.} & 10x10 & 10x20 & 10x30 & 20x20 & 20x30 &
30x30 \\\hline
$ \Prob{\E_{a}^{v} > 0}$ & 0.10 & 0.18 & 0.26 & 0.33 & 0.45 & 0.60 \\
    \hline
  \end{tabular*}
  \caption{\textbf{Probability of co-residency under the reference
      placement policy.}}
  \label{fig:ref-mode-prob}
\end{figure}


\begin{figure}
  \center
  \footnotesize
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline
    \textbf{Strategy} & $v$ \& $a$ & $a'$ & \textbf{Cost benefit} (\$) & \textbf{Normalized}\\
     & & & & \textbf{success}\\
    \hline
    S1 \& S2 & 10 & 688 & 113.87 & 10\\
    S3 & 30 & 227 & 32.75 & 1.67\\
    S4(i) & 20 & 105 & 4.36 & 2.67\\
    S4(ii) & 20 & 342 & 53.76 & 3.03\\
    S5 & 20 & 110 & 4.83 & 1.48\\
    \hline
  \end{tabular}
  \caption{\textbf{Cost benefit analysis.} $N = 1000$, $P(a_{type}) = 0.026$,
    which is the cost per instance-hour on EC2 (the cheapest). For
    simplicity $T_{d}(v,a) = (v * a) * 3.85$, where $3.85$ is fastest average
    time to detect co-residency per instance-pair. Here, $v \times a$ is the run
    configuration of the strategy under test. Note that the cost benefit is the
    additional cost incurred under the reference policy, hence is equal to cost
    incurred by $a'-a$ additional VMs.}
  \label{fig:cb-analysis}  
\end{figure}

Recall that a launch strategy in a cloud implies a placement vulnerability in
that cloud's placement policy if its normalized
success rate is greater than 1. The normalized success rate of the strategy
is the ratio of the chance of co-location under that launch strategy to the probability of
co-location in the reference policy ($\Prob{\E_{a}^{v} > 0}$). Below is a list
of selected launch strategies that escalate to placement vulnerabilities using
our reference policy with their normalized success rate in parenthesis.

%\begin{enumerate}
\begin{packeditemize}

\item[\textit{(S1)}] In Azure, launch ten attacker VMs closely after the
  victim VMs are launched (1.0/0.10).

\item[\textit{(S2)}] In EC2 and GCE, if there are known victims in
  any of the smaller datacenters, launch at least ten attacker VMs
  with a non-zero delay (1.0/0.10).

\item[\textit{(S3)}] In all three clouds, launch 30 attacker instances, either
  with no delay (Azure) or one hour delay (EC2, GCE) from victim launch, to get
  co-located with one of the 30 victim instances (1.00/0.60).

\item[\textit{(S4)}] (i) In Amazon EC2, launch 20 attacker VMs with
  a delay of 5 minutes or more after the victims are launched
  (0.88/0.33). (ii) The optimal delay between
  victim and attacker VM launches is around 4 hours for a 20x20 run (1.00/0.33).

\item[\textit{(S5)}] In Amazon EC2, launch the attacker VMs with
  1 hour after the victim VMs are launched where the time of day falls
  in the early morning, i.e., 02:00 to 10:00hrs PST 
  (0.89/0.60).
\end{packeditemize}
%\end{enumerate}

\paragraph{Cost benefit.} 
Next, we quantify the cost benefit of each of these strategies over the
reference policy. As the success rate of any launch strategy on a vulnerable
placement policy is greater than what is possible in the reference policy, 
we need more attacker instances in
the reference policy to achieve the same success rate. We
calculate this number of attacker instances $a'$ using: $ a' = \ln(1 -
S_{a}^{v})/\ln(1 - {v}/{N})$, where, $S_{a}^{v}$ is the success rate of a
strategy with run configuration of $v \times a$. The result of this calculation is
presented in~\figref{fig:cb-analysis}. The result shows that the best strategy,
S1 and S2, on all three cloud providers is \$114 cheaper than what is possible
in the reference policy. 
%Note that this cost benefit considers the cheapest
%pricing model for the reference policy, whereas in reality a more secure
%placement policy may demand more money to be practical. 

It is also evident that these metrics enable evaluating and comparing various
launch strategies and their efficacy on various placement policies both
on robust placements and attack cost. For example, note that although the
normalized success rate of {\em S3} is lower than {\em S4}, it has a higher cost
benefit for the attacker. 

%
% Add discuss about cost benefit of the strategies.
% As one can notice, the relative increase in the chance of co-residency
% is very high even under a conservative model. Considering the low cost
% of small instance types and the large number of servers typically
% deployed in these public clouds, it is safe to conclude that all these
% public clouds are still vulnerable to co-residency attacks.

\subsection{Limitations}

Although we exhaustively experimented with a variety of
placement variables, the results have limitations. One major
limitation of this study is the number of placement variables and the
set of values for the variables that we used to experiment. For
example, we limited our experiments with only one instance type, one
availability zone per region and used only one account for the victim
VMs. Although different instance types may exhibit different placement
behavior, the presented results hold strong for the chosen
instance type. The
only caveat that may affect the results is if the placement policy uses
account ID for VM placement decisions. Since, we experimented
with only one victim account (separate from the designated attacker
account) across all providers, these results, in the worst case, may
have captured the placement behavior of an unlucky victim account that
was subject to similar placement decisions (and hence co-resident) as
that of the VMs from the designated attacker account. 

Even though we ran at least 190 runs per cloud provider over a period
of 3 months to increase statistical significant of our results, we
were still limited to at most 9 runs per run configuration (with 3
runs per time of day).  These limitations have only minor bearing on
the results presented, if any, and the reported results are
significant and impactful for cloud computing security research.


==> uncoop-coresidency_ <==

\subsection{Co-residency Detection on Uncooperative Victims}
\label{ssec:uncoop-test}
Until now, we described a method to detect co-residency with a cooperative
victim. In this section, we look at a more realistic setting where an adversary
wishes to detect co-residency with a victim VM with accesses limited to only
public interfaces like HTTP or a key-value (KV) store's put-get interface. We show that the basic cooperative co-residency detection  can also be employed to detect co-residency with an
uncooperative victim in the wild.

%% \vnote{I prefer a better name than ``uncooperative'' victim, which
%%   does not have a negative connotation to refer to a common case
%%   scenario. Any ideas?}

\begin{figure}
\center
%\includegraphics[scale=0.50]{figures/web-app-architecture.pdf}
\includegraphics[scale=0.40]{figures/web-app-architecture.eps}
\caption{{\bf An example victim web application architecture.}}
    \label{fig:web-app-arch}
\end{figure}


\paragraph{Attack setting.}
Unlike previous attack scenarios, we assume the attacker has no access to the
victim VMs or its application other than what is permitted to any user on the
Internet. That is, the victim application exposes a well-known public interface
(e.g., HTTP, FTP, KV-store protocol) that allows incoming requests, which is also
the only access point for the attacker to the victim. The front end of this
victim application can range from caching or data storage services (e.g.,
memcached, cassandra) to generic webservers. We also assume that there may be multiple instances of this
front-end service running behind a load balancer.  Under
this scenario, the attacker wishes to detect co-location with one or more of
the front-facing victim VMs.

%% Under this scenario, if we show that an attacker could detect coresidency with
%% one of the front-facing victim VMs (for e.g., the webservers) with just the
%% openly accessible public interfaces (in this case, via HTTP), we bridge the gap
%% between knowing the launch strategy to actually exploiting it in the wild and
%% detecting coresidency with an uncooperative victim. This is assuming that either
%% the attacker can indirectly trigger victim instance launches or known when the
%% victim VMs are launched. As mentioned earlier, such an assumption is reasonable
%% considering most applications in the cloud have a predictable diurnal load
%% variation~\vnote{any citation for this?}.

\paragraph{Co-residency test.}
We adapt the memory tests used in previous section by running the memory-locking
sender in the attacker instance. For a receiver, we use the public interface
exposed by the victim by generating a set of requests that potentially makes the
victim VMs hit the memory bus. This can be achieved by looping through a large number
of requests of sizes approximately equal or greater than the size of the
LLC. This creates a performance side-channel that leaks co-residency
information. This receiver runs in an independent VM under the adversary's
control, which we call the co-residency detector.

%% We employed the same property of the memory-locking test (method 1)
%% in~\secref{ssec:corestest} -- creating memory bus contention using
%% unaligned atomic operations~\cite{wu2012whispers}. Like the prior
%% method, we ran the memory-locking sender~\figref{fig:mlock-code} on
%% the attacker VM that is potentially coresident with one of the victim
%% webservers. The only difference is that the receiver is replaced with
%% a set of HTTP request to the victim web application instead of a
%% memory-probing receiver that relies on direct access to the victim. We
%% used an off-the-shelf HTTP performance measurement utility called
%% \texttt{HTTPerf}~\cite{httperf} to design the receiver. The
%% performance degradation due to the memory-locking contention induced
%% by a co-resident attacker is leaked via the average request latency on
%% the receiver. Further investigation reveals that this performance
%% degradation is significant enough even when the requests are serviced
%% by multiple webservers behind a load balancer. In the rest of this
%% section, we show how we reliably detect coresidency using this
%% technique on an uncooperative Olio webserver victim in Amazon EC2.




\paragraph{Experiment setup.}
To evaluate the efficacy of this method, we
used the Olio multi-tier web application~\cite{olio-workload} that is
designed to mimic a social-networking application. We used an instance of this
workload from CloudSuite~\cite{cloudsuite2}. Although Olio
supports several tiers (e.g., memcached to cache results of database queries),
we configured it with two tiers as shown in~\figref{fig:web-app-arch}, with
each webserver and the database server running in a separate VM of type t2.small
on Amazon EC2. Multiple of these webserver VMs are configured behind a
HAProxy-based load balancer~\cite{haproxy} running in an m3.medium instance (for
better networking performance). The load balancer follows the standard
configuration of using round-robin load balancing algorithm with sticky client
sessions using cookies. We believe such a victim web application and its
configuration is a reasonable generalization of real world applications running
in the cloud.

For the attacker, we use an off-the-shelf HTTP performance measurement utility
called \texttt{HTTPerf}~\cite{httperf} as the receiver in the co-residency
detection test. This receiver is run inside a t2.micro instance (for free of
charge). We used a set of 212 requests that included web pages and web objects
(images, PDF files). We gathered these requests
using the access log of manual navigation around the web application from a web browser.

\paragraph{Evaluation methodology.}
We start with a known co-resident VM pair using the cooperative co-residency
detection method. We configure one of the VMs as a victim webserver VM and
launch four more VMs: two webservers, one database server and a load balancer,
all of which are not co-resident with the attacker VM. 

%% The load balancer required a
%% medium instance as a low-to-moderate network performance (supported by micro and
%% small instances) was insufficient to sustain trivial loads on the web
%% application without saturating the network bandwidth.

Co-residency detection starts by measuring the average request latency at the
receiver inside the co-residency detector for the baseline (with idle attacker)
and contended case with the attacker running the memory-locking sender. A
significant performance degradation between the baseline and the contended case
across multiple samples reveal co-residency of one of the victim VMs with the
attacker VM. On Amazon EC2, with the above setup we observed an average request
latency of $4.66$ms in the baseline case and a $10.6$ms in the memory-locked
case, i.e., a performance degradation of $\approx 2.3\times$.

\paragraph{Background noise.} The above test was performed when the victim web
application was idle. In reality, any victim in the cloud might experience constant or
varying background load on the system. False positives or negatives may occur
when there is spike in load on the victim servers. In such case, we use the same
solution as in~\secref{ssec:coop-test} --- alternating between measuring the idle
and the contended case.

In order to gauge the efficacy of the test under constant background load, we
repeated the above experiment with varying load on the victim. The result of
this experiment is summarized in~\figref{fig:uc-vary-load}. Counterintuitively,
we found that a constant load on the background server exacerbates the
performance degradation gap, hence resulting in a clearer signal of
co-residency. This is because running memory-locking on the co-resident attacker
increases the service time of all requests as majority of the requests rely on
memory bandwidth. This increases the queuing delay in the system and in turn
increasing the overall request latency. Interestingly, this aforementioned
performance gap stops widening at higher loads of 750 to 1000 concurrent users
as the system hits a bottleneck (in our case a network bottleneck at the load
balancer) even without running the memory-locking sender. Thus, detecting
co-residency with a victim VM that
is part of a highly loaded and bottlenecked application would be hard using this test.


\begin{figure}
\center
\includegraphics[scale=0.75]{figures/uncoop-vary-load}
\caption{{\bf Co-residency detection on an uncooperative victim.} The
  graph shows the average request latency at the co-residency detector
  without and with memory-locking sender running on the co-resident
  attacker VM under varying background load on the victim. Note that
  the y-axis is in log scale. The load is in the number of concurrent
  users, where each user on average generates 20 HTTP requests per
  second to the webserver.}
    \label{fig:uc-vary-load}
\end{figure}

\ignore{
\begin{figure}
\centering\
\footnotesize
  \begin{tabular}{|c|c|c|c|c|c|}
    \hline
    \textbf{Load}&\textbf{Thruput} & \multicolumn{3}{c|}{\textbf{Avg. CPU Util.} (\%)} & \textbf{N/w b/w} \\
    (users) & (ops/sec) & \textbf{WS} & \textbf{DB} & \textbf{LB} & (MB/s)\\
    \hline
    100 & 19.89 & 4 & 6 & 10 & 7.34\\
    250 & 49.99 & 10 & 13 & 24 & 18.48\\
    500 & 100.47 & 19 & 25 & 43 & 35.88\\
    750 & 151.78 & 27 & 38 & 52 & 53.58\\
    1000 & 181.42 & 31 & 45 & 54 & 64.18\\
\hline
\end{tabular}
\caption{}
\label{fig:olio-baseline}
\end{figure}
}

\begin{figure}
\center
\includegraphics[scale=0.75]{figures/uncoop-vary-server-load}
\caption{{\bf Varying number of webservers behind the load balancer.}  The graph
  shows the average request latency at the co-residency detector without and
  with memory-locking sender running on the co-residency attacker VM under
  varying background load on the victim. Note that the y-axis is in log
  scale. The error bars show the standard deviation over 5 samples.}
    \label{fig:uc-vary-server-load}
\end{figure}


We also experimented with increasing the number of victim webservers behind the
load balancer beyond 3 (\figref{fig:uc-vary-server-load}). As expected, the
co-residency signal grew weaker with increasing victims, and at 9
webservers, the performance degradation was too low to be useful for
detecting co-residency. 

%% \subsection{Limitations}
%% \paragraph{Discussion.}
%% \vnote{Tone up the discussion on limitations, the covert-channel
%%   signal is clear and is strong enough to be considered as the ground
%%   truth}

%% The limitation of our co-residency detection test is that it is
%% impossible to validate the veracity (or rate of false positives and
%% negatives) of these tests as we do not have access to the ground truth
%% about co-residency. That said, in the thresholding mechanism we make
%% sure that we either use a high threshold or use multiple tests before
%% detecting co-residency. Thus, the number of co-resident pairs detected
%% in this study could be safely considered as a lower bound on the
%% actual number of co-resident pairs.

